Non-linear extension of interval arithmetic and exact resolution of interval equations over square regions

The interval numbers is the set of compact intervals of $\mathbb{R}$ with addition and multiplication operation, which are very useful for solving calculations where there are intervals of error or uncertainty, however, it lacks an algebraic structure with an inverse element, both additive and multiplicative This fundamental disadvantage results in overestimation of solutions in an interval equation or also overestimation of the image of a function over square regions. In this article we will present a solution to this problem, through a morphism that preserves both the addiction and the multiplication between the space of the interval numbers to the space of square diagonal matrices.

==> name.tex <==
\begin{example}
Consider the following interval linear equation $[1,2]X+[3,6]=[3,8]$, suppose first that $X$ is non-negative, then we have the following matrix equation
\begin{align}
\left(\begin{array}{cc}
1 & 0 \\ 
0 & 2
\end{array}\right) X+\left(\begin{array}{cc}
3 & 0 \\ 
0 & 6
\end{array}\right)=
\left(\begin{array}{cc}
3 & 0 \\ 
0 & 8
\end{array}\right)
\end{align}
then the solution is
\begin{align}
  X=  \left(\begin{array}{cc}
0 & 0 \\ 
0 & 1
\end{array}\right) 
\end{align}
suppose now that $X$ is non-posotive, then we have the following matrix equation
\begin{align}
\left(\begin{array}{cc}
2 & 0 \\ 
0 & 1
\end{array}\right) X+\left(\begin{array}{cc}
3 & 0 \\ 
0 & 6
\end{array}\right)=
\left(\begin{array}{cc}
3 & 0 \\ 
0 & 8
\end{array}\right)
\end{align}
then the solution is
\begin{align}
  X=  \left(\begin{array}{cc}
0 & 0 \\ 
0 & 2
\end{array}\right) 
\end{align}
The first solution corresponds to a matrix whose first entry is less than or equal to the last entry, in addition to complying with our assumption of being non-negative for what represents an interval, however the second solution cannot represent any interval, since that X was considered negative and we obtained an interval that represents a positive interval. Therefore, the solution is $X=[0,1]$.
\end{example}
\begin{example}
 Consider the following equation $X(1-X)=[0,\frac{1}{4}]$ suppose first that $0\leq x\leq 1$, then under this condition we have   $\varphi(x)\varphi(1-X)=\left(\begin{array}{cc}
0 & 0 \\ 
0 & \frac{1}{4}
\end{array}\right)$  the result of this equation in interval is $X=\displaystyle\left[0,\frac{1}{2}+\frac{1}{\sqrt{2}}\right]$. 
\end{example}
\begin{example}
 The equation $X^2-X=[0,1]$ has no solution for $x\geq 0$, however calculating the image of the interval $\displaystyle\left[1,\frac{1}{2}+\frac{\sqrt{5}}{2}\right]$ under the function $f(x)=x^2-x$ we obtain $[0,1]$. This fact is due to the fact that the interval arithmetic does not distinguish intervals even when they are under the same symbol, that is, in taking a random value in $X ^ 2$ this is in general different than the value taken in $X$.
\end{example}
The general theory of equations intervalares resolution of the board in section \ref{resol}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Connection between intervals and matrices and a small problem}
We will introduce an application between the space of the intervals to the space of the diagonal square matrices. This application will play a role in extending the space of the intervals algebraically, to a commutative ring with unity, where we will have more degrees of freedom to solve equations or compute images on square regions, however, not always the solutions we obtain, in this space It will have an analogue as an interval.
\begin{definition}
Let $X=[x_1,x_2]\in K_c(\mathbb{R})$, then the interval conjugate to $X$ is $\widehat{X}=[x_2,x_1]$.
\end{definition}
 Let $X\in K_c(\mathbb{R})$, for simplication let's assume that $x_1$ is the smallest element  and $x_2$ is the largest element of $X$. For the next proposition we are going to defined the following subset of $K_c(\mathbb{R})$:
\begin{enumerate}
    \item $K_c(\mathbb{R})_0^+=\{X\in K_c(\mathbb{R}),x_1\geq 0\}$,
    \item $K_c(\mathbb{R})_0^-=\{X\in K_c(\mathbb{R}),x_2\leq 0\}$,
     \item $K_c(\mathbb{R})^+=\{X\in K_c(\mathbb{R}),x_1> 0\}$,
    \item $K_c(\mathbb{R})^-=\{X\in K_c(\mathbb{R}),x_2< 0\}$.
\end{enumerate}
\begin{proposition}\label{propro} Let $\varphi:Kc(\mathbb{R})\to \mathcal{D}_2(\mathbb{R})$ defined by  $\varphi([a,b])=\left(\begin{array}{cc}
a & 0 \\ 
0 & b
\end{array}\right)$. Then $\varphi$ satisfies the following properties:
\begin{enumerate}
    \item $\varphi(X+Y)=\varphi(X)+\varphi(Y)$ for all $X,Y\in Kc(\mathbb{R}) $,
    \item $\varphi(kX)=k\varphi(X)$ for all $X\in Kc(\mathbb{R})$ and $k\geq 0$,
    \item $\varphi(kX)=k\varphi(\widehat{X})$ for all $X\in Kc(\mathbb{R})$ and $k\leq 0$,
    \item $\varphi(XY)=\varphi(X)\varphi(Y)$ for all $X,Y\in Kc(\mathbb{R})_0^+ $,
    \item $\varphi(XY)=\varphi(X)\varphi(\widehat{Y})$ for all $X\in Kc(\mathbb{R})_0^- $ and $Y\in Kc(\mathbb{R})_0^+ $,
    \item $\varphi(XY)=\varphi(\widehat{Y}))\varphi(\widehat{Y})$ for all $X,Y\in Kc(\mathbb{R})_0^- $.
\end{enumerate}
\end{proposition}
\textbf{Proof} By simple inspection.
 \begin{flushright}
$ \blacksquare$
 \end{flushright}


We observe that the function is one to one, however it is not onto, since for a matrix to represent an interval we must have that the first entry must be less than or equal to the last entry, in this case we will say that the matrix represents an interval in the classical sense. This last condition is necessary and sufficient to guarantee the existence of the that the inverse image of $\phi$ is an interval. Since by restricting the range of phi to the set of matrices with this characteristic, we obtain a bijection.\\

From this application, we can solve linear linear equations, expressing them as a matrix equation, where we have more algebraic freedoms compared to the interval artimetic. However, not all the solutions we obtain from the matrix equations could be interval solutions, since if the solution we obtain does not satisfy the property of having the first entry less than or equal to the last entry, there is simply no interval solution for the interval equation. For example, the following equations have no solution in the set of intervals: $X+[a_1,a_2]=[0,0]$ and $X[a_1,a_2]=[1,1]$, and by applying the $\varphi$ function on these equations we get as solution $\varphi X=
\left(\begin{array}{cc}
-a_1 & 0 \\ 
0 & -a_2
\end{array}\right)$
and $\varphi X=
\left(\begin{array}{cc}
\displaystyle\frac{1}{a_1} & 0 \\ 
0 & \displaystyle\frac{1}{a_2}
\end{array}\right)$
 respectively. where we notice that the first entry is greater than or equal to the last entry, then there is no solution for the interval equation, as expected.
 
 
The proposition presents a compatibility problem between the different properties that it mentions in the proposition, for example, if we consider $X,Y\in Kc(\mathbb{R})^+$ and $Z\in Kc(\mathbb{R})^-$ such that $X+Z\in Kc(\mathbb{R})^-$, then  $\varphi(XY+ZY)$ , for (1),(4) and (5) is $\varphi(X)\varphi(Y)+\varphi(Z)\varphi(\widehat{Y})$, however we can also apply (5) on $\varphi((X+Z)Y)$ and We obey this $\varphi(X)\varphi(\widehat{Y})+\varphi(Z)\varphi(\widehat{Y})$. This problem of incompatibility between the properties is because they are incomplete. however in the interval arithmetic, this type of problem does not exist. In the next section we will solve this problem, stated a general result that we will call the Fundamental Theorem of Interval Functions and through this result we will state the fundamental theorem of Interval Equations
